Santal\'o Geometry of Convex Polytopes

The Santal\'o point of a convex polytope is the interior point which leads to a polar dual of minimal volume. This minimization problem is relevant in interior point methods for convex optimization, where the logarithm of the dual volume is known as the universal barrier function. When translating the facet hyperplanes, the Santal\'o point traces out a semi-algebraic set. We describe and compute this geometry using algebraic and numerical techniques. We exploit connections with statistics, optimization and physics.

==> SIAGA/ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Prevent itemized lists from running into the left margin inside theorems and proofs
\usepackage{enumitem}
\setlist[enumerate]{leftmargin=.5in}
\setlist[itemize]{leftmargin=.5in}

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{Santal\'o Geometry of Convex Polytopes}{D. Pavlov and S. Telen}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{Santal\'o Geometry of Convex Polytopes\thanks{Submitted to the editors \today.}}

% Authors: full names plus addresses.
\author{Dmitrii Pavlov\thanks{Max Planck Institute for Mathematics in the Sciences and TU Dresden (current) 
  (\email{pavlov@mis.mpg.de}).}
\and Simon Telen\thanks{Max Planck Institute for Mathematics in the Sciences 
  (\email{simon.telen@mis.mpg.de}).}}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 


==> SIAGA/response2 <==
RESPONSE TO REFEREE 2 OF "Santaló Geometry of Convex Polytopes"

We thank the referee for their insightful comments on our manuscript. We have addressed all of them and revised the paper accordingly. For the referee's convenience, we copied the comments below, together with a short reply to each of them. To this revision, we have also attached a pdf "diff.pdf" in which all changes are highlighted. 

Small comments to the authors are below: 

page 3, Example 1.2 -- "11 3-dimensional" -> "11 three-dimensional" 

REPLY: Fixed.

page 8, proof of Prop 2.5 -- Is there a reference for the notion of an "iterated residue"? It would also be nice to add half a sentence to the end of the proof justifying that $\gamma(b)$ cannot jump from +1 to -1. 

REPLY: We added a reference to Thomas Lam's introductory text on positive geometries for the notion of an iterated residue. The fact that $\gamma(b)$ is a constant (i.e. it does not depend on b), given as the ratio of the determinant of $W_{I(u)}$ to its absolute value, means that it cannot jump from -1 to +1. This is idependent of the choice of the vertex $u$: $\gamma(b)$ by definition can only depend on $b$, not on the choice of vertex of the polytope. The point of this part of the proof is to demonstrate that $\gamma$ actually does not depend on b.  

page 9, proof of Prop. 3.2 -- "\Sigma(b)" -> "\Sigma(B)" 

REPLY: Fixed.

page 14, proof of Prop. 4.3 -- It would be better to not use $x$ for both the subscript of the projection and the name of the point (e.g. $\pi_x^{-1}(x)$ is unfortunate). Perhaps you could use $\pi_1$ and $\pi_2$ for the projections instead of $\pi_x$ and $\pi_u$. Or use $x_0$ for the point (e.g. $\pi_x^{-1}(x_0)$) as you do later in the paper. 

REPLY: Done.

Also, "$n_c$" -> "$n_C$" 

REPLY: Fixed. 

page 15/16, Section 5 -- In the beginning of the section $M_{\C}$ is used for a variety in complex affine space. This is the context for the definition of ML degree. When $M_{\C}(Q)$ is introduced, it is a variety in projective space. It would be nice to be consistent with this. 

REPLY: We have made this consistent. 

page 16, Lemma 5.1 -- It would be nice to move "with $p_v$ from (22)" to the sentence before, in which $p_i$ is used. 

REPLY: We have stated Lemma 5.1 more clearly in the revision. 

page 19, Conjecture 5.7 -- I think it would be better to make two conjectures here and change the "sketch of proof" to a proof that one of the conjectures implies the other. 

REPLY: Done

page 19, Sketch of proof -- missing ")" in the sentence "What's missing ... ". 

REPLY: Fixed.

page 19, Example 5.8 -- I believe that all minors of a totally positive matrix are positive, not only the maximal ones. 

REPLY: this depends on the reference. We adopt the terminology used in the context of positive geometries. A totally positive matrix is a matrix representing an element of the totally positive Grassmannian (see e.g. Definition 2.4 in https://arxiv.org/abs/2110.10856v2), which means that only the maximal minors, resulting in Pluecker coordinates, are positive. 

page 20, Section 6 -- perhaps it would be better not to name the coordinates of $q$, since $q_1$ is used so heavily in the rest of the section. For example "$q = (q_1, \hdots, q_m)$" could instead be "$q \in \mathbb{C}^m$". 

REPLY: Fixed. 

page 21, line 3 -- Please add a word or two before $(A\cdot W = 0)$ so that it doesn't look like a single equation with the preceding $W$. 

REPLY: Done. 

page 23, Example 6.3 -- "$x_1^*(b_1)=$" -> "$x_1^*(b_1) \approx$" 

REPLY: Fixed. 

page 23, concluding discussions -- The use of $\epsilon$ vs. $\varepsilon$ is inconsistent. Also, the connection to linear programming (and beyond) could be made stronger. What do the authors view as the potential applications (in theory or practice) to linear programming? How does this barrier function compares with those more commonly used in linear programs. For example, is it self-concordant? Does it have some advantage? Is it plausible that the homotopy methods introduced here is competitive with other interior point methods?

REPLY: We agree with the referee that the connection to linear programming was not sufficiently elaborated on. We have added section 6.3, with a comment on self-concordance and an explicit example of how to use the volumetric barrier in interior point methods. We are hesitant to comment on competitiveness with other interior point methods, as this is not our expertise and requires future research. 


==> drdfwwsjcbdqjvbqqqqbxfhdqmybtfsy/SIAGA/ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Prevent itemized lists from running into the left margin inside theorems and proofs
\usepackage{enumitem}
\setlist[enumerate]{leftmargin=.5in}
\setlist[itemize]{leftmargin=.5in}

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{Santal\'o Geometry of Convex Polytopes}{D. Pavlov and S. Telen}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{Santal\'o Geometry of Convex Polytopes\thanks{Submitted to the editors \today.}}

% Authors: full names plus addresses.
\author{Dmitrii Pavlov\thanks{Max Planck Institute for Mathematics in the Sciences and TU Dresden (current) 
  (\email{pavlov@mis.mpg.de}).}
\and Simon Telen\thanks{Max Planck Institute for Mathematics in the Sciences 
  (\email{simon.telen@mis.mpg.de}).}}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 


==> drdfwwsjcbdqjvbqqqqbxfhdqmybtfsy/SIAGA/response2 <==
RESPONSE TO REFEREE 2 OF "Santaló Geometry of Convex Polytopes"

We thank the referee for their insightful comments on our manuscript. We have addressed all of them and revised the paper accordingly. For the referee's convenience, we copied the comments below, together with a short reply to each of them. To this revision, we have also attached a pdf "diff.pdf" in which all changes are highlighted. 

Small comments to the authors are below: 

page 3, Example 1.2 -- "11 3-dimensional" -> "11 three-dimensional" 

REPLY: Fixed.

page 8, proof of Prop 2.5 -- Is there a reference for the notion of an "iterated residue"? It would also be nice to add half a sentence to the end of the proof justifying that $\gamma(b)$ cannot jump from +1 to -1. 

REPLY: We added a reference to Thomas Lam's introductory text on positive geometries for the notion of an iterated residue. The fact that $\gamma(b)$ is a constant (i.e. it does not depend on b), given as the ratio of the determinant of $W_{I(u)}$ to its absolute value, means that it cannot jump from -1 to +1. This is idependent of the choice of the vertex $u$: $\gamma(b)$ by definition can only depend on $b$, not on the choice of vertex of the polytope. The point of this part of the proof is to demonstrate that $\gamma$ actually does not depend on b.  

page 9, proof of Prop. 3.2 -- "\Sigma(b)" -> "\Sigma(B)" 

REPLY: Fixed.

page 14, proof of Prop. 4.3 -- It would be better to not use $x$ for both the subscript of the projection and the name of the point (e.g. $\pi_x^{-1}(x)$ is unfortunate). Perhaps you could use $\pi_1$ and $\pi_2$ for the projections instead of $\pi_x$ and $\pi_u$. Or use $x_0$ for the point (e.g. $\pi_x^{-1}(x_0)$) as you do later in the paper. 

REPLY: Done.

Also, "$n_c$" -> "$n_C$" 

REPLY: Fixed. 

page 15/16, Section 5 -- In the beginning of the section $M_{\C}$ is used for a variety in complex affine space. This is the context for the definition of ML degree. When $M_{\C}(Q)$ is introduced, it is a variety in projective space. It would be nice to be consistent with this. 

REPLY: We have made this consistent. 

page 16, Lemma 5.1 -- It would be nice to move "with $p_v$ from (22)" to the sentence before, in which $p_i$ is used. 

REPLY: We have stated Lemma 5.1 more clearly in the revision. 

page 19, Conjecture 5.7 -- I think it would be better to make two conjectures here and change the "sketch of proof" to a proof that one of the conjectures implies the other. 

REPLY: Done

page 19, Sketch of proof -- missing ")" in the sentence "What's missing ... ". 

REPLY: Fixed.

page 19, Example 5.8 -- I believe that all minors of a totally positive matrix are positive, not only the maximal ones. 

REPLY: this depends on the reference. We adopt the terminology used in the context of positive geometries. A totally positive matrix is a matrix representing an element of the totally positive Grassmannian (see e.g. Definition 2.4 in https://arxiv.org/abs/2110.10856v2), which means that only the maximal minors, resulting in Pluecker coordinates, are positive. 

page 20, Section 6 -- perhaps it would be better not to name the coordinates of $q$, since $q_1$ is used so heavily in the rest of the section. For example "$q = (q_1, \hdots, q_m)$" could instead be "$q \in \mathbb{C}^m$". 

REPLY: Fixed. 

page 21, line 3 -- Please add a word or two before $(A\cdot W = 0)$ so that it doesn't look like a single equation with the preceding $W$. 

REPLY: Done. 

page 23, Example 6.3 -- "$x_1^*(b_1)=$" -> "$x_1^*(b_1) \approx$" 

REPLY: Fixed. 

page 23, concluding discussions -- The use of $\epsilon$ vs. $\varepsilon$ is inconsistent. Also, the connection to linear programming (and beyond) could be made stronger. What do the authors view as the potential applications (in theory or practice) to linear programming? How does this barrier function compares with those more commonly used in linear programs. For example, is it self-concordant? Does it have some advantage? Is it plausible that the homotopy methods introduced here is competitive with other interior point methods?

REPLY: We agree with the referee that the connection to linear programming was not sufficiently elaborated on. We have added section 6.3, with a comment on self-concordance and an explicit example of how to use the volumetric barrier in interior point methods. We are hesitant to comment on competitiveness with other interior point methods, as this is not our expertise and requires future research. 

